ARDIR: Improving Robustness using Knowledge Distillation of Internal Representation

Adversarial training is the most promising method for learning robust models against adversarial examples. A recent study has shown that knowledge distillation between the same architectures is effective in improving the performance of adversarial training. Exploiting knowledge distillation is a new approach to improve adversarial training and has attracted much attention. However, its performance is still insufficient. Therefore, we propose Adversarial Robust Distillation with Internal Representation~(ARDIR) to utilize knowledge distillation even more effectively. In addition to the output of the teacher model, ARDIR uses the internal representation of the teacher model as a label for adversarial training. This enables the student model to be trained with richer, more informative labels. As a result, ARDIR can learn more robust student models. We show that ARDIR outperforms previous methods in our experiments.

==> src/main_symbol.tex <==
\begin{table}[t]
\begin{center}
  \caption{Definition of main symbols}
  \scriptsize
  \begin{tabular}{|c|l|}
    \hline 
    Symbol & Definition \\ \hline \hline
    $\bm{x}$ & Input data. \\ \hline
    $\bm{y}$ & True Label \\ \hline
    $\bm{\eta}$ & Adversarial Perturbation. \\ \hline
    $\epsilon$ & Limitation of perturbation magnitude. \\ \hline
    $\phi_{\theta}$ & Deep Neural Network Model with parameterize $\theta$. \\ \hline
    $\phi_{\theta}(\bm{x})$ & Output when $x$ is input to $\phi_{\theta}$. \\ \hline
    $\phi_{\theta,l}(\bm{x})$ & $l$ layer output when $x$ is input to $\phi_{\theta}$. \\ \hline
    $l$ & layer of DNN Model. $l=1,2,\dots,L$ \\ \hline
    $W$ & Width of layer\\ \hline
    $H$ & Height of layer. \\ \hline
    $T$ & Teachar Model\\ \hline
    $\bm{x}^{T}$ & Teachar data \\ \hline
    $\sigma_{t}$ & Softmax with Temperature. \\ \hline
    $t$ & temperature constant. \\ \hline
    $\ell$ & Loss function\\ \hline
    $D$ & Distance between two intermediate output\\ \hline
    $KL$ & Kullback–Leibler divergence\\ \hline
    $\beta$ & hyperparameter in Proposed method \\ \hline
  \end{tabular}
  \label{symbol}
\end{center}
\end{table}
